SPHERE/ZIMPOL insights into discs around evolved stars: arcs, asymmetries and dust properties

Second-generation circumbinary discs around evolved binary stars, such as post-Asymptotic Giant Branch (post-AGB) binaries, provide insights into poorly understood mechanisms of dust processing and disc evolution across diverse stellar environments. We present a multi-wavelength polarimetric survey of five evolved binary systems - AR Pup, HR 4049, HR 4226, U Mon, and V709 Car - using the Very Large Telescope SPHERE/ZIMPOL instrument. Post-AGB discs show significant polarimetric brightness at optical and near-IR wavelengths, often exceeding 1% of the system's total intensity. We also measured a maximum fractional polarisation of the scattered light for AR Pup of ~0.7 in the V-band and ~0.55 in the I-band. To investigate wavelength-dependent polarisation, we combine the SPHERE/ZIMPOL dataset with results from previous SPHERE/IRDIS studies. This analysis reveals that post-AGB discs exhibit a grey to blue polarimetric colour in the optical and near-IR. Along with high fractional polarisation of the scattered light and polarised intensity distribution, these findings are consistent with a surface dust composition dominated by porous aggregates, reinforcing independent observational evidence for such grains in post-AGB circumbinary discs. We also find evidence of diverse disc geometries within the post-AGB sample, including arcs, asymmetries and significant variations in disc size across optical and near-IR wavelengths for some systems (U Mon, V709 Car). On comparing post-AGB discs to circumstellar environments around AGB stars and YSOs, we found that post-AGB systems exhibit a higher degree of polarisation than single AGB stars and are comparable to the brightest protoplanetary discs around YSOs.

==> Null.tex <==
%Table 2

\begin{landscape}
    \begin{table}
        \caption{Photometric data of the targets. See text for full details.}
        \begin{center}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{ c c c c c c c c c c c c c c c c c c c c c }
            \hline
            Object Name & RA ($\degree$) & Dec ($\degree$) & U & B & SDSS.RP & V & R & I & J & H & K & W1 & W2 & AKARI.S9W & IRAS.F12 & W3 & W4 & IRAS.F25 & IRAS.F60 & IRAS.F100\\
            \hline
            J005107  & 12.780083 & -73.692598 & 16.65 & 16.657 & 99.99 & 15.84 & 15.45 & 14.85 & 14.33 & 13.65 & 12.93 & 11.39 & 10.44 & 99.99 & 99.99 & 8.365 & 6.926 & 99.99 & 99.99 & 99.99 \\
            MACHO 47.2496.8  & 73.930267 & -67.852718 & 17.31 & 16.23 & 99.99 & 15.08 & 14.28 & 14.00 & 13.19 & 12.67 & 12.57 & 12.09 & 11.79 & 99.99 & 99.99 & 10.26 & 9.248 & 99.99 & 99.99 & 99.99 \\
            HD 158616 & 262.695520 & -11.368968 & 11.92 & 10.09 & 9.368 & 9.642 & 99.99 & 99.99 & 7.845 & 7.299 & 6.525 & 5.178 & 4.029 & 3.301 & 3.520 & 2.600 & 1.234 & 2.900 & 1.600 & 1.980 \\
            V453 Oph  & 261.704705 & -2.393453 & 12.29 & 11.90 & 10.30 & 10.85 & 10.50 & 9.791 & 8.806 & 8.442 & 8.283 & 7.993 & 7.890 & 99.99 & 99.99 & 7.743 & 7.549 & 99.99 & 99.99 & 99.99 \\
            \hline
            \end{tabular}
            }
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The RA and DEC coordinates are given for the J2000 epoch. Null magnitudes are listed as 99.999.
        \end{tablenotes}
       
        \label{tab:photometry}
    \end{table}    ,
\end{landscape}




%Table 1

\begin{landscape}
    \begin{table}
        \caption{This table lists the object name and alternative widely used name for each object in the sample along with two sets of stellar parameters. The final column lists the references to the literature analysis.}
        \begin{center}
            \begin{tabular}{ c l l c c c c c c c c c c  }
                \hline
            \#ID & Object Name & Other Name & \begin{tabular}[c]{@{}l@{}}\Teff\\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & & \begin{tabular}[c]{@{}l@{}}\Teff \\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & Ref. \\
                \hline
        		\multicolumn{3}{ c }{} & \multicolumn{4}{c }{This Study} & \multicolumn{5}{c }{Literature} \\
                \hline
                1 & J005107.19-734133.3 &	OGLE SMC-T2CEP-18	& 5768 $\pm$ 100	&	0.21 $\pm$ 0.10	&	-1.57 $\pm$ 0.10   &	4.08 $\pm$ 0.50	& & 5267 $\pm$ 250	&	0.72 $\pm$ 0.50	&	-1.56 $\pm$ 0.50  & ... & 1	\\
                2 & MACHO 47.2496.8 &	OGLE LMC-T2CEP-15	&
                4898 $\pm$ 100	&	0.00 $\pm$ 0.50	&	-1.42 $\pm$ 0.16   &	4.00 $\pm$ 1.00	& & 4900 $\pm$ 250	&	0.00 $\pm$ 0.50	&	-1.50 $\pm$ 0.50   &	3.50 $\pm$ 1.00  &	2\\
                3 & HD 158616 &	IRAS 17279-1119	& 7379 $\pm$ 110	&	1.47 $\pm$ 0.25	&	-0.50 $\pm$ 0.20   &	2.97 $\pm$ 0.25 &  & 7250 $\pm$ 125	&	1.25 $\pm$ 0.25	&	-0.64 $\pm$ 0.12 &	3.00 $\pm$ 0.50 &	3\\
                4 & V453 Oph &	BD-02 4345	& 	6158 $\pm$ 100	&	1.19 $\pm$ 0.25	&	-2.27 $\pm$ 0.10   &	2.50 $\pm$ 0.50 &  & 6250 $\pm$ 250	&	1.50 $\pm$ 0.50	&	-2.23 $\pm$ 0.12   &	3.00 $\pm$ 0.50 & 4\\
                \hline
            \end{tabular}
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The stellar parameters under "This study" represent the spectroscopically determined atmospheric parameters obtained using the $Python$ wrapper of i-Spec whereas the stellar parameters under the title "Literature" represent the spectroscopically determined atmospheric parameters from the Literature analysis. Note that the low-resolution spectral analysis of J005107.19-734133.3 did not provide an estimated \mv value. Detailed information on the tabulated information can be found in the individual studies identified in column 'Ref'. The column 'Ref.' indicates the individual study: 1 - \cite{Kamath2014}, 2 - \cite{Reyniers2007}, 3 - \cite{desmedt2016}, 4 - \cite{Deero2005}\\
        \end{tablenotes}
       
        \label{tab:sample}
    \end{table}    ,
\end{landscape}


==> chap_paper3.tex <==
\chapter{Diversity of second-generation protoplanetary discs with SPHERE multi-wavelength polarimetric imaging}\label{ch:paper3}
\graphicspath{{ch_paper3/}} 


\clearpage

\textit{This chapter was originally prepared for publication as:}\\
\textbf{Revealing the diversity of second-generation discs around evolved stars with multi-wavelength high-resolution polarimetric imaging from SPHERE.}\\
K. Andrych, D. Kamath, H. Van Winckel, H. M. Schmid, J. Milli, J. Kluska \\
\textit{Monthly Notices of the Royal Astronomical Society}, in prep.\\
\\
\textit{This chapter presents the multi-wavelength polarimetric imaging results for five post-AGB binary systems—AR Pup, HR 4049, HR 4226, U Mon, and V709 Car—obtained with SPHERE/ZIMPOL and SPHERE/IRDIS (when available) across optical ($V-$ and $I-$bands) and near-IR ($H$-band) wavelengths. Building on the methodology developed in Chapters~\ref{ch:paper1} and \ref{ch:paper2}, we apply a systematic approach to investigate wavelength-dependent dust scattering and polarization properties in this diverse sample. This study represents the most extensive high-resolution polarimetric imaging analysis of post-AGB circumbinary discs to date, and the results are currently being prepared for publication.} \\
\\
\textbf{\textit{Author Contributions}}\\
K. Andrych performed the data reduction and analysis of SPHERE multi-wavelength polarimetric data presented in this chapter. D.\,Kamath and H.\,Van Winckel provided feedback and engaged in regular discussions throughout each stage of the research process. H.\,M.\,Schmid and J.\,Milli contributed to the data reduction. J.\,Kluska and D.\,Kamath are the principal investigators of the proposals that resulted in the data used in this study. The chapter was written by K.\,Andrych, with D.\,Kamath providing feedback and comments.

% Abstract of the paper
\begin{tcolorbox}[colback=blue!10!white, boxrule=0mm]
    \section{Original paper abstract}
    Investigating second-generation circumbinary discs around evolved binary stars, such as post-Asymptotic Giant Branch (post-AGB) binaries, provides insights into the poorly understood processes behind dust formation and binary interactions that end the giant evolutionary phase of these stars. This study examines the polarimetric properties, surface morphologies, and dust characteristics of circumbinary discs in post-AGB systems across optical and near-infrared wavelengths, presenting multi-wavelength polarimetric imaging of five post-AGB binary systems (AR Pup, HR 4049, HR 4226, U Mon, and V709 Car) obtained with the Very Large Telescope/SPHERE instrument at the European Southern Observatory. Our results show high polarimetric disc brightness ($\geq$1\%), grey to blue polarimetric colours, and intensity distributions in post-AGB circumbinary discs, suggesting porous dust aggregates as the main dust composition. For one post-AGB system, AR\,Pup, we directly measured a maximum polarization efficiency of $\sim$0.7 in the $V-$band and $\sim0.55$ in the $I'-$band. One system in our sample, V709\,Car, shows a distinctly larger polarimetric emission in the $I'$-band than in the $V$-band and clumpy, less confined polarimetric emission compared to post-AGB discs. These findings align with the suggestion that V709 Car may be less evolved, with its primary star potentially still in the AGB evolutionary stage. The results of this study strengthen parallels between circumbinary discs around post-AGBs and protoplanetary discs around YSOs, such as complex morphologies, high polarimetric brightness, and wavelength-dependent behaviour, highlighting post-AGB systems as valuable models for disc evolution across stellar environments.
    
\end{tcolorbox}

\section{Introduction}
\label{sec:paper3_intro}

At the end of their lives, low- to intermediate-mass stars (0.8-8M$_\odot$) experience significant mass loss as they evolve along the asymptotic giant branch (AGB). This mass loss plays a key role in the chemical enrichment of the interstellar medium, although the details of the mass-loss process are not yet fully understood \citep{Habing2003agbs.conf.....H, Khouri2020A&A...635A.200K}. In binary systems, mass loss can be amplified through stellar interactions, often resulting in the formation of dusty circumbinary discs during the post-AGB phase \citep{VanWinckel2003ARA&A..41..391V, Kamath2015MNRAS.454.1468K, Bertolami2016A&A...588A..25M}. Studying these second-generation circumbinary discs around post-AGB binary stars provides insights into the still-mysterious processes that govern dust formation and the binary interactions that terminate the giant evolutionary phase of these stars.

Observational studies have revealed key parameters regarding the structure and dynamics of circumbinary discs in post-AGB systems. These binary stars display a distinctive spectral energy distribution (SED) profile, with dust emission peaking in the near-infrared \citep[near-IR, e.g.,][]{DeRuyter2006A&A...448..641D, VanWinckel2009A&A...505.1221V, Kamath2014MNRAS.439.2211K, Kamath2015MNRAS.454.1468K, Gezer2015MNRAS.453..133G, Kluska2022}. Such near-IR excess is typically attributed to circumstellar dust and gas within a stable, compact disc with an inner rim near the dust sublimation radius. These discs are generally found to exhibit Keplerian rotation, with angular sizes ranging from roughly 0.5'' to 1'' (100 to 500 AU) as inferred from $^{12}{\rm CO}$ position-velocity mappings \citep[e.g.,][]{Bujarrabal2015A&A...575L...7B, Gallardo_cava2021A&A...648A..93G}. High-resolution near-IR interferometric studies have spatially resolved the hot dust inner rim in post-AGB discs, verifying that it is predominantly located at dust sublimation radius \citep[$\sim$6\,AU; e.g.,][]{Hillen2016, Kluska2019A&A...631A.108K}. These circumbinary discs are called 'full discs'. However, the recent study by \citet{Corporaal2023A&A...674A.151C} confirmed the presence of 'transition' post-AGB discs with the dust inner rim up to 7.5 times larger than the theoretical dust sublimation radius. Pilot high-resolution imaging studies of 9 post-AGB circumbinary discs with VLT/SPHERE revealed their complex morphologies and large diversity in terms of disc size and orientation \citep{Ertel2019AJ....157..110E, Andrych2023MNRAS.524.4168A}. The latter study also identified significant polarized brightness of post-AGB circumbinary discs in near-IR wavelengths, reaching up to $2\%$ of the total system intensity. Recently, a detailed multi-wavelength polarimetric imaging study of the post-AGB binary IRAS\,08544-4431 revealed a relatively consistent polarized brightness across optical and near-IR wavelengths, along with substantial forward scattering in optical polarimetry. These results align with theoretical models that propose large, porous aggregates of submicron-sized monomers as the main dust components. Furthermore, \citet{Andrych2024IRAS08} observed wavelength-dependent variations in the extended structure of the IRAS\,08544-4431 disc, with near-IR $H-$band observations showing a more extended disc surface than optical $V$ and $I-$bands. Authors suggest that this structural variation across wavelengths could indicate potential disc warping. Moreover, the presence of circumbinary disc significantly influences the chemical composition of the post-AGB binaries, often leading to a phenomenon known as photospheric chemical depletion of refractory elements 
\citep[\text{usually traced with [Zn/Ti]; i.e.,}][]{Mohorian2024MNRAS.530..761M}. This depletion arises from the re-accretion of chemically fractionated gas and dust in the circumbinary disc, resulting in unique elemental abundance patterns observed in these systems \citep{Oomen2019A&A...629A..49O, Kluska2022, Mohorian2024MNRAS.530..761M}. Furthermore, the impact of the circumbinary disc on the post-AGB binary system leads to a wide range of orbital parameters, including eccentricities and orbital periods. Long-term radial velocity monitoring studies show that the typical orbital periods of post-AGB binaries can range from a hundred to a few thousand days \citep{Oomen2018, VanWinckel2009A&A...505.1221V}.


Despite distinct formation histories and lifetimes, post-AGB circumbinary discs \citep[with a lifetime of $\sim10^4-10^5$ years,][]{Bujarrabal2017A&A...597L...5B} and protoplanetary discs (PPDs) around young stellar objects (YSOs) (with a lifetime of up to a few Myr) share many characteristics. Both disc types show comparable IR excesses, dust disc masses \citep[$\sim10^{-3}M_\odot$,][]{Corporaal_IRAS08_2023A&A...671A..15C}, chemical depletion patterns \citep{Kluska2022, Mohorian2024MNRAS.530..761M}, dust mineralogy \citep{Gielen2011A&A...533A..99G, Scicluna2020MNRAS.494.2925S}. They also exhibit similar polarimetric brightness and morphology \citep{Andrych2023MNRAS.524.4168A, Andrych2024IRAS08}. Moreover, radiative transfer (RT) modelling efforts for circumbinary discs around post-AGB binaries \citep[e.g.,][]{Corporaal_IRAS08_2023A&A...671A..15C} show that high-angular resolution interferometric data for these systems can be accurately reproduced by using passively irradiated disc models initially developed for PPDs around YSOs.


In this paper, we present multi-wavelength polarimetric imaging results for five post-AGB binary systems (AR\,Pup, HR\,4049, HR\,4226, U\,Mon, and V709\,Car) observed with VLT/SPHERE. We aim to investigate the consistency of polarimetric properties, surface morphologies, and dust composition across the post-AGB sample and to compare these with findings from AGB and YSO systems. In Section \ref{sec:paper3_target}, we present our target sample and relevant observational details collected from the literature. In Section \ref{sec:paper3_data}, we introduce our observing strategy and data reduction methodology. In Section~\ref{sec:paper3_analysis}, we present the analysis of the VLT/SPHERE-ZIMPOL data and corresponding results. In Section~\ref{sec:paper3_discussion}, we discuss the dust properties of post-AGB circumbinary discs and highlight similarities and differences between circumstellar environments of AGBs, circumbinary discs around post-AGBs, and PPDs around YSO. In Section~\ref{sec:paper3_conclusion}, we present our conclusions.


\section{Target details}
\label{sec:paper3_target}

In this study, we focus on five binary systems with known circumbinary discs: AR\,Pup, HR\,4049, HR\,4226, U\,Mon and V709\,Car. These targets were selected from the mid-infrared interferometric survey for discs around 19 post-AGB stars using VLTI/MIDI \citep{Hillen2017}.  The final selection was based on objects that are feasible for Spectro-Polarimetric High-contrast Exoplanet REsearch/Zurich Imaging Polarimeter \citep[$R_{mag}<11$; SPHERE/ZIMPOL,][]{Schmid2018A&A...619A...9S} and have inner warm disc diameters greater than 40 mas. Initially, all targets were classified as post-AGB binary stars based on their strong IR excesses in the SEDs, typically attributed to circumstellar dust near the dust sublimation temperature \citep{DeRuyter2006A&A...448..641D}. We note that the effective temperature T$_{\rm eff}$ derived from SED fitting for V709\,Car is $3500\pm175$ K, suggesting that this M-type star is too cool for a post-AGB object and may still be in the AGB phase \citep{Hillen2017, Kluska2022}. However, a detailed spectroscopic analysis is required to accurately determine its evolutionary stage. In this paper, we will refer to V709\,Car as a post-AGB object. 

This selection represents a diverse subset of five post-AGB binary systems, offering insights into disc properties and evolutionary stages across different circumstellar environments. SEDs of the targets, together with near- and mid-IR interferometric data, suggest a variety of disc orientations and characteristics \citep{Hillen2017, Kluska2019A&A...631A.108K}. Some systems, like HR\,4049, are seen nearly face-on, while others, such as AR\,Pup, are edge-on and obscure their host stars. According to the classification of post-AGB discs by \citet{Kluska2022}, based on SED and IR-excess features, three out of five studied post-AGB systems (AR\,Pup, HR\,4049, U\,Mon) fall into the "full disc" category, while HR\,4226 and V709\,Car remain uncategorized. Furthermore, the sample spans a wide range of photospheric depletion of refractory elements (see Section~\ref{sec:paper3_intro}), with AR\,Pup and HR\,4049 exhibiting strong depletion ([Zn/Ti] > 1.5), while U\,Mon shows no depletion ([Zn/Ti] = 0). In Table\,\ref{tab:paper3_sample}, we present selected observational parameters of our target sample relevant to this study, including their corresponding IRAS names, Gaia DR3 distances, SED characteristics, orbital parameters, and interferometric disc sizes. In summary, our target sample displays diverse properties, particularly regarding atmospheric parameters of the primary star and binary orbital characteristics. By analyzing the polarimetric and interferometric data for these systems, we aim to provide a comprehensive understanding of how binary interactions influence the circumstellar environments of evolved stars.


\input{ch_paper3/Table1}


\section{Data and Observations}
\label{sec:paper3_data}

In this paper, we present multiwavelength, high-angular-resolution polarimetric observations of the circumbinary discs surrounding a sample of five post-AGB binary systems. This section provides an overview of the data and the methodology used for data reduction.

\subsection{Observations}
\label{sec:paper3_observations}

The data were obtained using the Zurich Imaging Polarimeter \citep[ZIMPOL,][]{Schmid2018A&A...619A...9S} of the extreme AO instrument SPHERE \citep{Beuzit2019}. For two targets (HR\,4049 and U\,Mon) we also adopted results of near-IR polarimetric observations using the Infra-Red Dual-beam Imaging and Spectroscopy camera \citep[IRDIS,][]{Dohlen2008} of the same instrument \citep{Andrych2023MNRAS.524.4168A}. In Table~\ref{tab:paper3_disc_orient}, we summarise the resulting disc parameters determined from IRDIS data as well as the results of this study (see Section~\ref{sec:paper3_analysis} for details).

The SPHERE/ZIMPOL data for this study were obtained as part of ESO observational program 0101.D-0752(A) (PI: Kamath). Observations were conducted as follows: AR\,Pup and HR\,4226 in April 2018, V709\,Car in May 2018, U\,Mon in December 2018, and HR\,4049\footnote{We note that HR\,4049 was observed twice, on the 7th and 8th of January 2019, due to improper observing conditions during the first observation.} in January 2019. To effectively resolve the scattered light around the post-AGB binary stars and ensure the best accuracy for the multi-wavelength characteristics, we used SPHERE/ZIMPOL in its polarimetric P1 mode without coronagraph. This mode provides high polarimetric sensitivity and calibration accuracy by averaging out instrumental effects as the sky field rotates with respect to the instrument and telescope pupil \citep{Schmid2018A&A...619A...9S}. In addition to the target systems, we observed reference stars (HD71253, HD75885, HD96314, HD94680, and HD98025) selected for their similar brightness, colour, and location to the corresponding binary systems. These reference stars were observed immediately after each target, allowing their data to serve as a point-spread function (PSF) during the reduction process.

We obtained data in both the $V$-band and $I'$-band for all targets in our sample. For the $V$-band, we used the ZIMPOL 'V' filter ($\lambda_0 = 554$\,nm, $\Delta\lambda = 80.6$\,nm). For the $I'$-band, we used the ZIMPOL 'Cnt820' filter ($\lambda_0 = 817.3$\,nm, $\Delta\lambda = 19.8$\,nm) for HR\,4049, HR\,4226, and U\,Mon, and the ZIMPOL 'N\_I' filter ($\lambda_0 = 816.8$\,nm, $\Delta\lambda = 80.5$\,nm) for AR\,Pup and V709\,Car. For the convenience of the reader, while the exact ZIMPOL filter names are specified in the tables throughout the paper, we will refer to both 'Cnt820' and 'N\_I' as the $I'$-band in the text and figures. Due to the design of the ZIMPOL camera, observations in both $V$-and $I'$-bands for each target were taken simultaneously, enabling direct comparison of data during further analysis. The data were taken in polarimetric cycles, where one cycle includes four Stokes exposures for linear polarization measurements, with half-wave plate positions $\theta = 0^{\circ}$ and $45^{\circ}$ for Stokes Q and $\theta = 22.5^{\circ}$ and $67.5^{\circ}$ for Stokes U. In total 20 polarimetric cycles were taken for each target and 10 polarimetric cycles for reference stars. Each observational frame contained $\sim10^{5}-10^{6}$ counts, ensuring non-saturated observations \citep{Schmid2018A&A...619A...9S}. 


\subsection{Data reduction}
\label{sec:paper3_data_reduction}

The reduction of our SPHERE/ZIMPOL polarimetric data was performed using the methodology outlined in \citet{Andrych2024IRAS08}. Initial steps, including bias subtraction, flat fielding, frame centring, polarimetric beam shift correction, and calculation of the Stokes vectors $Q$ and $U$, were carried out using the High-Contrast Data Centre (HC-DC, formerly SPHERE Data Centre) pipeline\footnote{This software is based on the SPHERE ESO pipeline, complemented with additional routines such as improved centring algorithms, automatic frame sorting, and analysis tools for systematic SPHERE data processing.} \citep{Delorme2017sf2a.conf..347D}. 

To correct our data for polarization induced by the instrument, we used the $sz$-pipeline developed at ETH Zurich. This pipeline, following the methodology outlined by \citet{Schmid2018A&A...619A...9S}, calculates the offset in telescope polarization and polarization position angle for the ZIMPOL instrument. In Appendix~\ref{sec:paper3_ap_telesc_corr}, we provide details of the measured fractional polarization ($Q/I_{\rm tot}, U/I_{\rm tot}$, where $I_{\rm tot}$ is the total intensity of the target) before and after correction for each observation cycle, alongside the corresponding telescope polarization data for each target.

Further processing included our custom Python pipeline. To account for frame-to-frame variability caused by atmospheric conditions, we selected the best 75\%\footnote{This value was selected to balance between excluding frames with poorer instrumental performance while still keeping enough frames to benefit from mean combining and significantly improve the signal-to-noise ratio.} of frames based on the normalized peak intensity $I_{\rm tot}$. Then, we computed azimuthal Stokes parameters $Q_\phi$ and $U_\phi$ (following the definitions of \citet{deBoer2020}), total polarized intensity $I_{\rm pol}$, and the Angle of Linear Polarization $AoLP$. Positive $Q_\phi$ indicates linear polarization in the azimuthal direction, while negative $Q_\phi$ indicates radial polarization. $U_\phi$ represents linear polarization shifted by $\pm45^\circ$ from the azimuthal and radial directions. The AoLP indicates the orientation of the polarization vector in each region of the polarized image.

For low-inclination ($i \lesssim 40^\circ$) and optically thick discs (assuming single scattering of stellar light on the disc surface), the polarization vectors of scattered light are expected to align azimuthally with respect to the central star \citep{Canovas2015A&A...582L...7C}. This allows to adopt $Q_\phi$ as the measure of polarized flux and to avoid bias effects from noisy observational data, compared to the polarized intensity $I_{\rm pol}$, which is derived as $\sqrt{Q^2 + U^2}$ \citep{Simmons1985A&A...142..100S}. To test this approach for our data, we calculated the ratio of total azimuthally polarized signal $Q_\phi$ to $I_{\rm pol}$. We found that azimuthally polarized intensity accounts for over 85\% of the total polarized intensity $I_{\rm pol}$ in both the $V$- and $I'$-bands for HR\,4049 and HR\,4226, indicating the dominance of single scattering. For AR\,Pup, the azimuthally polarized intensity is lower, around 75\% in the $V$-band and 80\% in the $I'$-band, likely due to the disc’s nearly edge-on orientation. In U\,Mon and V709\,Car, the fraction is even lower ($\sim57\%$ and $\sim68\%$ in the $V$-band, and $\sim65\%$ and $\sim80\%$ in the $I'$-band, respectively), likely due to higher disc inclinations and potential multiple scattering, which alters the polarization vector orientation. Additionally, we examined the mean flux distribution in $U_\phi$ across radial annuli, similar to the analyses by \citet{Avenhaus2018ApJ...863...44A, Andrych2023MNRAS.524.4168A}. While all targets showed signs of astrophysical signal in $U_\phi$, it is challenging to distinguish between residual instrumental effects and true physical signal. For all targets except HR\,4049 we found that the net $U_\phi$ signal accounts for more than 5\% of $Q_\phi$, supporting the use of $I_{\rm pol}$ for further analysis. For HR\,4049, however, we will use $Q_\phi$.

The reduced linearly polarized images of all targets show features commonly attributed to the polarized signal from the bright but spatially unresolved central region of the circumbinary disc \citep[e.g.,][]{Keppler2018A&A...617A..44K}. These features include a butterfly pattern in the central part of the $Q_\phi$, as well as a halo in the polarized total intensity image (see top row of Fig.~\ref{fig:paper3_ap_reduct_AR_pup},\,\ref{fig:paper3_ap_reduct_HR4049},\,\ref{fig:paper3_ap_reduct_HR4226},\,\ref{fig:paper3_ap_reduct_umon},\,\ref{fig:paper3_ap_reduct_v709} in Appendix~\ref{sec:paper3_ap_reduct}). To correct the data for the polarized signal from the bright, unresolved central region, we applied the method from \citet{Holstein2020A&A...633A..64V}. We used a circular aperture with a radius of 3 pixels ($\sim11$ mas)\footnote{Similar to \citet{Andrych2023MNRAS.524.4168A}, the 3-pixel aperture was chosen to reliably correct for the unresolved polarized signal while minimizing contributions from the resolved signal.} centred on the stellar position to calculate the degree and angle of the unresolved central polarization for all targets (see Table~\ref{tab:paper3_unresolved}). We also compare the DoLP of the unresolved polarization component (see Table ~\ref{tab:paper3_disc_orient} and Section~\ref{sec:paper3_data_reduction} for details) with the total linear polarization detected from reference stars at the observed wavelengths (see Fig.~\ref{fig:paper3_wave_dep_unres}). This comparison helps determine whether the unresolved signal primarily originates from interstellar polarization or the disc itself. While interstellar polarization has minimal effect on the total resolved polarization from a disc surface, it is included in the measured unresolved central polarization. Since stellar light is generally expected to be mostly unpolarized, and the reference stars were selected within $15^\circ$ of the corresponding targets, we use the reference star polarization as an estimate of the interstellar polarization along the line of sight. We found that for HR\,4049 and V709\,Car the DoLP of of the unresolved polarization component closely aligns with the estimated interstellar polarization. In contrast, for AR\,Pup, HR\,422, and U\,Mon, the DoLP of the unresolved polarization is significantly higher, indicating that it is primarily driven by the unresolved portion of the circumbinary disc rather than the polarization from the diffuse interstellar medium along the line of sight. We also note that in the case of AR\,Pup, viewed nearly edge-on with the disc partially obscuring the central star, the unresolved central polarized signal is overestimated, making it impossible to subtract without disturbing the resolved disc structure. For all other targets, we subtracted the measured unresolved central polarized signal from the $Q$ and $U$ images and recalculated $Q_\phi$ and $I_{\rm pol}$, ensuring that the final images reflect only the resolved circumstellar material. This method, however, produces unrealistically low intensity in the central 5x5 pixel region of the $I_{\rm pol}$ and $Q_\phi$ images, and any intrinsic $Q_\phi$ component remains undetectable due to limited spatial resolution. Therefore, we exclude this region from further analysis, noting that this discrepancy is an artefact of the reduction process. The resulting polarized images are presented in Fig.\ref{fig:paper3_reduced}. We also note that the reduced $I_{\rm pol}$ for HR\,4226, HR\,4049, and V709\,Car exhibits a thin cross-shaped decrease in polarized intensity, particularly visible in the $V$-band data for HR 4226. This pattern is not a genuine feature but rather a reduction artefact, as it is also seen in reference star data for these targets. While the exact cause of this effect is unclear, we emphasize that it is not a physical characteristic of the circumbinary discs of HR 4226, HR 4049, and V709\,Car.

\begin{figure} 
    \includegraphics[width=0.49\linewidth]{SourcesPlots/reduction/unres_DOLP_with_ref.png}
    \includegraphics[width=0.495\linewidth]{SourcesPlots/reduction/AoLP_wavelendep.png}
    \caption[Characteristics of unresolved central polarization for scientific targets and polarized intensity of reference stars as a function of wavelength.]{Characteristics of unresolved central polarization for scientific targets and polarized intensity of reference stars as a function of wavelength. The top panel shows the degree of unresolved polarization (solid lines) relative to the total intensity of each target and the polarized intensity relative to the total intensity for each reference star (dashed lines). The bottom panel displays the corresponding orientation of unresolved polarization (AoLP) for the targets (solid lines) and reference stars (dashed lines). Each target binary system and its corresponding reference star are indicated by matching colours. See Section~\ref{sec:paper3_data_reduction} for more details.}
    \label{fig:paper3_wave_dep_unres}
\end{figure}

To accurately estimate the total polarized flux of the disc, we have also corrected resolved $Q_\phi$ and $I_{\rm pol}$ images for polarimetric cancellation due to PSF smearing. This smearing appears due to the convolution of the Stokes $Q$ and $U$ with the instrument PSF. Following the methodology proposed by \citet{Ma2024A&A...683A..18M} to obtain corrected or intrinsic values for disc polarized intensity, we derived a two-dimensional correction map for the azimuthally polarized disc intensity $Q_\phi$ based on the observational PSF and disc orientation for each target. We adopted the inclination and position angle of the disc for each system (see Table~\ref{tab:paper3_sample}) from previous polarimetric imaging \citep[if available,][]{Ertel2019AJ....157..110E,Andrych2023MNRAS.524.4168A} or IR interferometric studies \citep{Hillen2016}. To ensure accurate wavelength dependant comparison of SPHERE/ZMPOL and SPHERE/IRDIS data, we have also calculated similar correction maps for the $H-$band SPHERE/IRDIS data for HR\,4049 and U\,Mon that were already analysed and presented by \citet{Andrych2023MNRAS.524.4168A}. We note that correction maps rise sharply within $\sim50$ mas from the central binary where PSF smearing causes significant polarimetric cancellation of the disc signal. While this correction is crucial for restoring total polarimetric brightness in small angular discs, it can distort the resolved disc structure near the binary. Therefore, while it was applied to restore the total polarimetric brightness, this correction was excluded when determining the disc's orientation and morphology.

To determine the statistically significant region of the final reduced images, we followed a method similar to that used for SPHERE observations of IRAS\,08544-4431 \citep{Andrych2024IRAS08}. In brief, we first calculated the background noise by analyzing an annular region of the reduced $I_{\rm pol}$ image free of the target signal and determined the pixel-to-pixel root mean squared. Using the calculated SNR, we then defined the region of $I_{\rm pol}$ with SNR $\geq 3$ as statistically significant for each observation (see second and fourth column of Fig.~\ref{fig:paper3_reduced}), which was then used for further analysis. We also evaluated the data resolution to compare with the expected SPHERE/ZIMPOL performance. Using Gaussian fitting of the PSF intensity profile, we measured the full width at half maximum (FWHM) as the resolution element size. We found a resolution of $\sim 30$ mas for all targets except AR\,Pup, which is consistent with SPHERE/ZIMPOL specifications \citep{Schmid2018A&A...619A...9S}. For AR\,Pup, the resolution was around 40 mas, likely due to slightly worse observing conditions or suboptimal selection of the reference star used for the PSF reference.

Finally, to retrieve disc substructures we deconvolved the resulting linearly polarized images with the reference PSF using the Richardson–Lucy deconvolution algorithm \citep{Richardson1972JOSA...62...55R, Lucy1974AJ.....79..745L}. We note that convergence of the deconvolution process was achieved within 30 iterations for both $V-$ and $I'-$bands for all targets, with pixel-to-pixel variation between neighbouring iterations reaching less than 1.5\%. However, we note that the same amount of iterations was overcorrecting the AR\,Pup and V709\,Car images, resulting in degenerate results. Therefore, for AR\,Pup and V709\,Car, we stopped iterations when we achieved pixel-to-pixel variation of 5\% ($\sim10$ iterations).


\input{ch_paper3/Table2}

\begin{figure}
    
    \includegraphics[width=0.98\linewidth]{SourcesPlots/reduction/PI_reduced+deconv.png}
    \caption[Total polarized intensity of all targets in $V-$ and $I'-$bands.]{Total polarized intensity of all targets in $V-$ and $I'-$bands. The first and third columns display reduced polarimetric images without PSF deconvolution, while the second and fourth columns show images after the deconvolution process. White contours outline regions of statistically significant polarized intensity (SNR=3). White circles in the lower-left corner of each image indicate the size of the resolution element. All images are presented on an inverse hyperbolic scale and oriented North up and East to the left. See Section~\ref{sec:paper3_data_reduction} for more details.}
    \label{fig:paper3_reduced}
\end{figure}


\section{Analysis and Results}
\label{sec:paper3_analysis}

In this section, we present the analysis of reduced linearly polarized images and discuss the results for each target individually, following the methodology presented in \citet{Andrych2024IRAS08}. Our analysis includes investigating the fractional polarization, determining the disc orientation, defining the relative disc brightness in polarized light, and characterizing the wavelength-dependent polarized intensity and structure of circumbinary discs.


\subsection{Investigating variations in aperture polarimetry}
\label{sec:paper3_aper_pol}

To investigate geometric variations in the circumbinary discs of our five targets, we analyzed how fractional polarization ($Q/I_{\rm tot}, U/I_{\rm tot}$) varies with distance from the central binary. This method offers insights into the unresolved disc component contributing to the detected central polarization. Significant tearing or misalignment in the disc would manifest as abrupt shifts in the $Q/I_{\rm tot}-U/I_{\rm tot}$ plane. 

We measured total fractional polarization $Q/I_{\rm tot}$ and $U/I_{\rm tot}$ using circular apertures that gradually increased in radius from 0.004'' to 0.11'' (0.25'' for AR\,Pup), with a step size of 0.0036'' (1 pixel). The resulting data (see Fig.~\ref{fig:paper3_aper_pol}) show a smooth and continuous change in fractional polarization with aperture size for all targets. However, the curves for AR\,Pup, HR 4226, and U\,Mon exhibit a more complex shape, likely due to changes in the orientation of the scattering surface relative to the binary, which affects the resulting polarization vector. Additionally, interstellar polarization contributes to the unresolved central polarization, impacting the fractional polarization closer to the binary. This effect could explain the changes in polarization orientation, particularly for HR 4226 and U\,Mon, given their small disc sizes. We discuss these factors in more detail for each target in Section~\ref{sec:paper3_indiv_cases}.

\begin{figure} 

    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/apperture/AR_Pup_dc_notnorm_QU_colored.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/apperture/HR4049_combined_QU_colored.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/apperture/HR4226_QU_colored.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/apperture/UMon_Katya_QU_colored.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/apperture/V709_Car_QU_colored.png}

    \caption[Fractional polarization $Q/I_{\rm tot}$ and $U/I_{\rm tot}$ for a gradually enlarging aperture for both $V-$ and $I'-$bands for all targets.]{Fractional polarization $Q/I_{\rm tot}$ and $U/I_{\rm tot}$ for a gradually enlarging aperture for both $V-$ and $I'-$bands for all targets. See Section~\ref{sec:paper3_aper_pol} for more details.}
    \label{fig:paper3_aper_pol}
\end{figure}

\subsection{Measuring the polarized disc brightness}
\label{sec:paper3_ polarised_bright}

To estimate the polarized disc brightness relative to the total intensity of the system, we calculated the ratio of the resolved polarized emission from the disc to the total unpolarized intensity of the target. The resolved polarized emission was measured within an area defined by a signal-to-noise ratio (SNR) of $\geq3$. To minimize bias, we used the azimuthal polarize, total polarized and unpolarized images (($Q_{\phi}$, $I_{\rm pol}$ and $I_{\rm tot}$) prior to deconvolution with the point spread function (PSF), while also accounting for the effects of PSF smearing during the observations (see Section \ref{sec:paper3_data_reduction}). We note that the resulting values for polarized disc brightness represent a lower limit due to the partial subtraction of the disc signal during data reduction. The final polarized disc brightness ratios ($Q_{\phi}/I$ and $I_{\rm pol}/I$) for both the $V-$ and $I'-$bands across all targets are presented in Table \ref{tab:paper3_disc_orient}. For reference, we also provide the polarized disc brightness value without PSF smearing correction ($I^{*}_{\rm pol}/I$).

To ensure an accurate comparison of the available SPHERE/ZIMPOL and SPHERE/ IRDIS data for our targets, we also applied a similar correction for PSF smearing to the $H$-band SPHERE/IRDIS data of HR\,4049 and U\,Mon, which were previously analyzed and presented by \citet{Andrych2023MNRAS.524.4168A}.

\input{ch_paper3/Table3}
 
\subsection{Determination of disc orientation}
\label{sec:paper3_disc_orient}

The final reduced polarized images reveal a clear bright 'ring' structure in both $V-$ and $I'-$band observations for HR\,4049, HR\,422, U\,Mon and V709\,Car (see Fig.~\ref{fig:paper3_reduced}). However, for V709\,Car, the "ring" is not fully resolved and exhibits lower polarized intensity compared to the other targets (see Section\ref{sec:paper3_ polarised_bright}), so it should be interpreted with caution. Additionally, no "ring" is observed for AR\,Pup due to the nearly edge-on disc orientation (see Sec.~\ref{sec:paper3_target} for details). Although we refer to the resolved structure as a 'ring,' it is important to clarify that the 'inner rim' in these images does not correspond to the physical dust inner rim of the circumbinary disc for any of the targets, as it is too small to be resolved by the SPHERE instrument. The unrealistically low intensity at the centre of the polarized image is caused by the correction of the unresolved polarization during data reduction (see Section \ref{sec:paper3_data_reduction}). Therefore, the bright 'ring' represents the smallest resolved section of the circumbinary disc close to the central binary and serves as a key indicator for determining the disc's position angle (PA) and inclination.

Following the methodology outlined in \citet{Andrych2023MNRAS.524.4168A, Andrych2024IRAS08}, we used the deconvolved linearly polarized images ($I_{\rm pol}$ or $Q_\phi$ for HR\,4049, see Section~\ref{sec:paper3_data_reduction}) to estimate the orientation of the resolved disc surface. To do this, we fitted an ellipse to the positions of peak brightness along the 'ring', from which we derived the lengths of the major and minor axes and the corresponding position angle (PA)\footnote{The PA was defined as rising counterclockwise from the vertical axis (North) to the first principal radius (major axis). We note that the ellipse fitting procedure allows the $180^{\circ}$ ambiguity in the disc PA on the sky.} of the disc.

Near-infrared interferometric observations of post-AGB circumbinary discs \citep[e.g.,][]{Kluska2018A&A...616A.153K, Corporaal2023A&A...674A.151C} indicate that the dust inner rim aligns with the dust sublimation radius (or even located further out), rather than being shaped by dynamical truncation from the inner binary. Therefore, regardless of the binary orbit eccentricity, we can assume the disc to be circular and interpret the visible elliptical disc shape (see second and fourth column of Fig.~\ref{fig:paper3_reduced}) as resulting from the projection of the circular disc onto the field of view. Thus, we can estimate the corresponding inclination that would cause this effect using:
\begin{equation}
    \cos{i}=(\frac{b}{a}),
	\label{eq:paper3_i}
\end{equation}
where $a, b$ are major and minor half axes of the ellipse.

The most plausible position and orientation of circumbinary discs, resolved in $V$ and $I'-$bands for each target, are presented in Fig.~\ref{fig:paper3_ellipse_fit} and Table~\ref{tab:paper3_disc_orient}. 

\begin{figure} 
     \includegraphics[width=0.26\linewidth]{SourcesPlots/analysis/ellipsefit/HR4049_combined_V_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/HR4226_V_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/UMon_Katya_V_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/V709_Car_V_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.26\linewidth]{SourcesPlots/analysis/ellipsefit/HR4049_combined_I_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/HR4226_I_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/UMon_Katya_I_ellipse_gauss_fit_all.jpeg}
     \includegraphics[width=0.24\linewidth]{SourcesPlots/analysis/ellipsefit/V709_Car_I_ellipse_gauss_fit_all.jpeg}
    
    \caption[Disc orientation results based on the polarimetric images of all targets.]{Disc orientation results based on the polarimetric images of all targets (see Section~\ref{sec:paper3_disc_orient} for more details). The red ellipses illustrate the most plausible PA and inclination of discs, while the dashed orange line highlights a significant substructure for HR\,4049 (see Section~\ref{sec:paper3_substr}). The red cross in the centre of the images represents the centre of the fitted ellipse, while the white cross represents the position of the binary. The low intensity of the central 5x5 pixel region of each image is a reduction bias caused by over-correction of the unresolved central polarization (Section~\ref{sec:paper3_data_reduction}). Note: all images are presented on an inverse hyperbolic scale.}
    \label{fig:paper3_ellipse_fit}
\end{figure}




\subsection{Exploring the extended disc morphology}
\label{sec:paper3_morphology}

In this section, we investigate the extended disc morphology of our targets by analyzing the disc brightness profiles and examining the resolved substructures in both the $V-$ and $I'-$bands.

\subsubsection{Brightness profiles}
\label{sec:paper3_profiles}

To explore the complexity of the resolved disc surface and reveal the spatial distribution of polarized intensity, we calculated linear, azimuthal, and radial brightness profiles following the methodology of \citet{Andrych2023MNRAS.524.4168A, Andrych2024IRAS08}. The brightness profiles for each target are presented in Appendix~\ref{sec:paper3_ap_profiles}, with individual discussions in Section~\ref{sec:paper3_indiv_cases}.

The linear brightness profiles reflect the symmetry of the disc along its major and minor axes (see Section~\ref{sec:paper3_disc_orient} for the details on determining disc orientation). These profiles for each target are shown in the top row of Fig.~ \ref{fig:paper3_profiles_hr4049},\,\ref{fig:paper3_profiles_hr4226},\,\ref{fig:paper3_profiles_umon},\,\ref{fig:paper3_profiles_v709car},\,\ref{fig:paper3_profiles_ar_pup}. We note that for AR\,Pup we use the estimation of the disc midplane orientation to define the position of major and minor axes (see Section~\ref{sec:paper3_ar_pup} for details).

The azimuthal brightness profile reflects asymmetries along the smallest resolved part of the circumbinary disc ('ring'). It was computed using bi-linear interpolation of the intensity from the four nearest pixels along the fitted ellipse in the linearly polarized image (see Section~\ref{sec:paper3_disc_orient}). This profile traces variations in azimuthal brightness starting from the eastern end of the major axis and proceeding counterclockwise. We note that we do not calculate azimuthal brightness profiles for AR\,Pup because it does not show an elliptical 'ring' (see Section~\ref{sec:paper3_disc_orient} for more details). The resulting brightness profiles are presented in the middle row of Fig.~\ref{fig:paper3_profiles_hr4049}, \ref{fig:paper3_profiles_hr4226}, \ref{fig:paper3_profiles_umon} for HR\,4049, HR\,4226 and U\,Mon, respectively.

The radial brightness profile describes the variation of scattered polarized emission with distance from the central binary. To account for the impact of disc orientation on the radial intensity distribution, we first reconstructed a 'face-on' view of the disc based on the estimated inclination of the resolved disc surface for both the $V-$ and $I'-$bands (see Section~\ref{sec:paper3_disc_orient} for details on the inclination and \citet{Andrych2023MNRAS.524.4168A} for more information on the methodology).
The deprojected polarized images were then subdivided into annuli, with widths increasing proportionally to $\sqrt{r}$, where $r$ is the corresponding radius. Finally, to plot the radial brightness profile, we calculated the mean brightness per pixel for these radially tabulated annuli, focusing only on statistically significant regions based on the SNR (see Section~\ref{sec:paper3_data_reduction}). To estimate the uncertainty, we used the variance of the pixel values in the same annuli of the $U_\phi$ image. Although this method overestimates the noise if any astrophysical signal is present in the $U_\phi$ image (which is the case for all targets in our sample, see Section\ref{sec:paper3_data_reduction}), it still allows us to establish an upper limit. The resulting deprojected polarized images and radial brightness profiles are presented in the bottom row of Fig.~\ref{fig:paper3_profiles_hr4049}, \ref{fig:paper3_profiles_hr4226}, \ref{fig:paper3_profiles_umon} for HR\,4049, HR\,4226 and U\,Mon respectively. We also plot similar profiles for AR\,Pup and V709\,Car; however, we do not perform the deprojection for these targets (Fig.~\ref{fig:paper3_profiles_v709car}, \ref{fig:paper3_profiles_ar_pup}). 


\subsubsection{Detection of substructures}
\label{sec:paper3_substr}

To detect and characterize potential substructures in the circumbinary disc, we adopted a qualitative analysis methodology similar to that described in \citet{Andrych2023MNRAS.524.4168A, Andrych2024IRAS08}. Our goal was to identify real features in the linearly polarized images (such as arcs or gaps) by combining the estimated SNR, the orientation of the polarization vector (AoLP), and the brightness of the disc substructures. 

First, we targeted regions of statistical significance in the linearly polarized images based on the calculated SNR ($\geq3$ for the final deconvolved polarimetric images). Next, we focus on the resolved substructures with a centrosymmetric distribution of polarization vectors, confirming that the polarimetric signal predominantly arises from the single scattering of stellar light on the disc surface. We present the local angles of linear polarization over the resolved structures in the deconvolved $I_{\rm pol}$ ($Q_\phi$ for HR\,4049, see Section~\ref{sec:paper3_data_reduction}) images for all targets in Fig.~\ref{fig:paper3_aolp} of Appendix~\ref{sec:paper3_ap_aolp}. 

Using these criteria, we identified reliable substructures in addition to the bright elliptic 'ring' in the polarimetric images of the circumbinary disc for all targets in both the $V$ and $I'-$bands. To quantify the brightness of these substructures, we calculated the percentage of total polarized intensity corresponding to the extended disc substructures and the central ring, excluding the unresolved central polarization (as shown in Fig.~\ref{fig:paper3_substr}). Notably, the substructures appear brighter in the $I'-$band compared to the $V-$band for all targets.


\begin{sidewaysfigure} 
     \includegraphics[width=0.21\linewidth]{SourcesPlots/analysis/substructures/HR4049_combined_Q_phi_V_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/HR4226_Q_phi_V_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/UMon_Katya_PI_V_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/V709_Car_PI_V_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/AR_Pup_dc_notnorm_PI_V_substr_perc_deconv.png}

     
     \includegraphics[width=0.21\linewidth]{SourcesPlots/analysis/substructures/HR4049_combined_Q_phi_I_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/HR4226_Q_phi_I_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/UMon_Katya_PI_I_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/V709_Car_PI_I_substr_perc.png}
     \includegraphics[width=0.19\linewidth]{SourcesPlots/analysis/substructures/AR_Pup_dc_notnorm_PI_I_substr_perc_deconv.png}
    
    \caption[Percentage of total polarized disc intensity per resolved structure for all targets in $V-$ and $I'-$bands.]{Percentage of total polarized disc intensity per resolved structure for all targets in $V-$ (top row) and $I'-$ (bottom row) bands (see Section~\ref{sec:paper3_substr}). All images are presented on an inverse hyperbolic scale and oriented North up and East to the left. The low intensity of the central 5x5 pixel region of each image is a reduction bias caused by over-subtracting of unresolved central polarization (Section~\ref{sec:paper3_data_reduction}).}
    \label{fig:paper3_substr}
\end{sidewaysfigure}


\subsection{Disc scattering morphology}
\label{sec:paper3_scatter}

The total intensity frames ($I_{\rm tot}$) for each target in the sample include both the stellar intensity and scattered light from the disc. To assess whether disentangling these components is feasible for our binary systems, we computed radial brightness profiles for the total intensity ($I_{\rm tot}$) of each post-AGB system and its corresponding reference single star (see Section~\ref{sec:paper3_profiles} for methodology details). The resulting profiles were normalized to the maximum intensity of each target. For four out of five targets (HR\,4049, HR\,422, U\,Mon, and V709\,Car), the radial intensity profiles closely match those of the reference star, indicating that the image is strongly dominated by the variable PSF of the star. The small angular size of the resolved discs makes their intensity too weak to detect. However, this is not the case for AR\,Pup. The radial brightness profile for $I_{\rm tot}$ of AR\,Pup is less steep than that of the reference star (see Fig.~\ref{fig:paper3_scattered}). In this system, the disc partially obscures the central binary (see Section~\ref{sec:paper3_data} and Fig.~\ref{fig:paper3_reduced}), improving the contrast and allowing the disc to be resolved in total intensity.

\begin{figure} 
     \includegraphics[width=0.49\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_V_scattered.png}
     \includegraphics[width=0.49\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_I_scattered.png}
  
    \caption[Radial profiles of normalized total intensity ($I_{\rm tot}/I^{\rm max}_{\rm tot}$) for AR\,Pup and reference star HD\,75885.]{Radial profiles of normalized total intensity ($I_{\rm tot}/I^{\rm max}_{\rm tot}$) for AR\,Pup (orange circles) and reference star HD\,75885 (blue squares), and normalized polarized intensity ($I_{\rm pol}/I^{\rm max}_{\rm pol}$) for AR\,Pup (green stars). See Section~\ref{sec:paper3_scatter} for details.}
    \label{fig:paper3_scattered}
\end{figure}

Moreover, we can compute the Degree of Linear Polarization (DoLP) map of the resolved scattered emission by calculating the pixel-to-pixel ratio of polarized intensity to the total intensity of the system ($I_{\rm pol}/I_{\rm tot}$). Since the disc of AR\,Pup obscures the central binary, we are unable to disentangle the direct stellar light from the scattered disc component using the method suggested by \citet{Tschudi2021A&A...655A..37T}. They demonstrated that disc intensity can be separated from stellar signal when the disc displays a bright, narrow ring located far enough from the star. In this case, a combination of the reference star's intensity profile and the disc's polarized intensity profile can be used for fitting.
For AR\,Pup, however, the total intensity ($I_{\rm tot}$) near the binary is dominated by direct stellar light, leading to non-detectable polarimetric efficiency at the centre of the derived DoLP map (see Fig.~\ref{fig:paper3_AR_Pup}). 

To carefully retrieve the scattered morphology of the disc we also deconvolve the resulting $I_{\rm tot}$ and DoLP map of AR\,Pup with observational PSF (see Section~\ref{sec:paper3_data_reduction} for details).
The final deconvolved total intensity image and DoLP map of AR\,Pup in $V-$ and $I'-$bands are presented in Fig.~\ref{fig:paper3_AR_Pup}. These results are further discussed in Section~\ref{sec:paper3_ar_pup}. 

\subsection{Wavelength-dependent polarized intensity and structure of circumbinary disc}
\label{sec:paper3_wavelength}

\begin{figure} 
    
    \includegraphics[width=0.48\linewidth]{SourcesPlots/analysis/wavelength/qphi_vs_pi_after_smearing.png}
    \includegraphics[width=0.495\linewidth]{SourcesPlots/analysis/wavelength/pi+-smearing.png}
    \caption[Polarized disc brightness as a function of wavelength for all targets.]{Polarized disc brightness as a function of wavelength for all targets. The top panel shows azimuthal ($Q_{\phi}/I$, dashed line) and total ($I_{\rm pol}/I$, solid line) polarized disc brightness relative to the total intensity of each target. The bottom panel shows total polarized disc brightness before ($I^{*}_{\rm pol}/I$, dashed line) and after ($I_{\rm pol}/I$, solid line) correction for the PSF smearing (see Section~\ref{sec:paper3_data_reduction}). See Section~\ref{sec:paper3_wavelength} for more details.}

    \label{fig:paper3_wave_dep}
\end{figure}

Polarimetric observations provide an estimate of the amount of light polarized by the disc surface layers, thereby offering a lower limit for the reflected light from the disc surface \citep[e.g.,][]{Benisty2022arXiv220309991B}. However, accurately characterizing dust in distant post-AGB circumbinary discs through polarimetry is challenging due to factors like small angular disc size, instrumental limitations, and uncertainties in the disc's geometry. Despite these challenges, we can measure the total polarized brightness of the disc across different wavelengths. Assuming similar scattering geometries across these wavelengths, the observed differences in the polarized signal are primarily caused by the scattering and absorption properties of the dust in the disc. Therefore, the wavelength dependence of the polarized brightness is a valuable indicator for studying the dust properties \citep[e.g.,][]{Ma2023A&A...676A...6M, Ma2024A&A...683A..18M}. 

To establish the wavelength dependence of the disc polarized intensity, we combined results from this study in the $V$ and $I'-$bands with available SPHERE/IRDIS $H-$band observations for HR\,4049 and U\,Mon \citep{Andrych2023MNRAS.524.4168A}. It is important to note that the disc polarized brightness discussed in \citet{Andrych2023MNRAS.524.4168A} was not corrected for PSF smearing effects (see Section~\ref{sec:paper3_data_reduction}). Therefore, we applied an additional correction to the $H-$band polarimetric results to ensure a consistent comparison of the disc polarized brightness across the $V-$, $I'-$, and $H-$bands. The wavelength dependence of the disc total ($I_{\rm pol}/I$) and azimuthal ($Q_{\phi}/I$) polarized intensity for each target system is shown in the top panel of Fig.~\ref{fig:paper3_wave_dep}. We note that for U\,Mon, $I_{\rm pol}/I$ decreases more steeply with wavelength than $Q_{\phi}/I$, though this does not affect the overall trend for the target. For all other systems, $I_{\rm pol}/I$ and $Q_{\phi}/I$ overlap within the uncertainties.

To quantitatively assess the wavelength dependence of the polarized disc brightness, we calculate the logarithmic gradient of the polarized intensity between two wavelengths, which serves as a measure of disc polarimetric colour:

\begin{equation}
    \eta_{\lambda_2/\lambda_1}=\frac{\rm log(Q_\phi/I_{tot})_{\lambda_1}-log(Q_\phi/I_{tot})_{\lambda_2}}{\rm log(\lambda_2/\lambda_1)},
	\label{eq:paper3_color}
\end{equation}

where $\lambda_1 < \lambda_2$, and $-0.5 < \eta < 0.5$ is classified as grey colour, $\eta < -0.5$ as blue and $\eta > 0.5$ as red  \citep{Tazaki2019MNRAS.485.4951T, Ma2023A&A...676A...6M}.

The resulting optical ($\eta_{V/I}$) and optical-IR ($\eta_{V/H}$) polarimetric colour for each target binary system are presented in Table~\ref{tab:paper3_disc_orient}. Notably, three out of the five post-AGB systems (HR\,4049, HR\,422, V709\,Car, and AR\,Pup) exhibit results consistent with a grey disc colour, while U\,Mon and HR\,4049 display borderline blue colour.



\begin{figure} 
    \centering
    \includegraphics[width=0.7\linewidth]{SourcesPlots/analysis/wavelength/colors_pi.png}

    \caption[Polarimetric colour indices (logarithmic wavelength gradients) $\eta$ for the disc polarized brightness.]{Polarimetric colour indices (logarithmic wavelength gradients) $\eta$ for the disc polarized brightness for all targets from this study and post-AGB binary IRAS\,08544-4431 \citep{Andrych2024IRAS08}. Black points are colours $\eta_{VH}$ between $V-$ and $H-$bands, and orange points for $\eta_{VI}$ between $V-$ and $I'-$bands. The shading represents the used definition of blue, grey, and red disc polarimetric colour. See Section~\ref{sec:paper3_wavelength} for details.}
    \label{fig:paper3_color}
\end{figure}

To examine how PSF smearing affects the wavelength dependence of the disc polarized intensity, we overplotted the total polarized intensity before ($I^{*}_{\rm pol}/I$) and after PSF correction ($I_{\rm pol}/I$) (see the bottom panel of Fig.~\ref{fig:paper3_wave_dep}). As discussed in Section~\ref{sec:paper3_data_reduction}, the PSF smearing correction increases sharply closer to the central binary. Due to the higher resolution and finer pixel scale of SPHERE/ZIMPOL observations in the $V$- and $I'-$bands compared to SPHERE/IRDIS in the $H$-band, this results in a more substantial correction of the polarized disc brightness in the optical than in the near-IR. We also note that PSF smearing has a greater impact on discs with emission concentrated closer to the central binary than on those with more extended emission. 

A multi-wavelength polarimetric imaging study of the post-AGB system IRAS\,08544-4431 revealed variations in disc size and morphology across different wavelengths \citep{Andrych2024IRAS08}. To investigate whether similar effects are present in our targets, we first compared the morphology of the smallest resolved section of the circumbinary disc close to the central binary (the bright 'ring'). Unlike the results for IRAS\,08544-4431, we did not find any significant variation (beyond the uncertainty) in the apparent inclination of the discs with wavelength (see Fig.\ref{fig:paper3_ellipse_fit} and Table~\ref{tab:paper3_disc_orient}).

We also combined polarimetric images of all our targets in the $V$ and $I'-$band data (from this study), along with $H-$band data for HR\,4049 and U\,Mon (adapted from \citet{Andrych2023MNRAS.524.4168A}). The $I_{\rm pol}$ images ($Q_\phi$ for HR\,4049, see Section~\ref{sec:paper3_data_reduction}) were normalized to the corresponding total intensity of the target. In Fig.~\ref{fig:paper3_combined} we present the final combined polarimetric images of all target systems in the $V$, $I'$, and $H-$bands (when available). To emphasize the intensity changes along the disc, we applied an inverse hyperbolic scale and a discrete colour map. We note that substructures are more pronounced in the $I'-$band compared to the $V-$band for HR\,4049, AR\,Pup, and HR\,422, but a noticeable difference in disc size is observed only for V709\,Car, where the disc appears more extended in the $I'-$band. Additionally, while comparing SPHERE/ZIMPOL optical results with SPHERE/IRDIS near-IR images, we found that U\,Mon shows a more extended disc in the near-IR, whereas HR\,4049 does not exhibit any change in size. We further discuss the results for each binary system individually in Section~\ref{sec:paper3_indiv_cases}.


\begin{figure*} 
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/combined/HR4049_combined_all_q_phi_discret.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/combined/HR4226_all_pi_discret.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/combined/UMon_Katya_all_pi_discret.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/combined/V709_Car_all_pi_discret.png}
    \includegraphics[width=0.32\linewidth]{SourcesPlots/analysis/combined/AR_Pup_dc_notnorm_all_pi_discret.png}
    
    \caption[Combined $Q_\phi$ multi-wavelength polarized disc morphology for all targets.]{Combined $Q_\phi$ polarized disc morphology for all targets using $V$ and $I-$band data from this study, along with the SPHERE/IRDIS $H-$band results for HR\,4049 and U\,Mon (adopted from \citet{Andrych2023MNRAS.524.4168A}). The black cross represents the position of the binary star. Before combining the $Q_\phi$ images in each band, they were normalized to the total intensity. In addition, we also provide the results of the geometric modelling of mid-IR ($N-$band) interferometric data for the full disc systems in our sample. The red circle represents the disc size obtained by \citet{Kluska2019A&A...631A.108K} for near-IR observations with VLTI/PIONIER instrument and the white circle represents the disc sublimation radius and outer disc size obtained by \citet{Hillen2017} for mid-IR with VLT/MIDI. Images are presented on an inverse hyperbolic scale and normalized to highlight the intensity change along the discs. See Section~\ref{sec:paper3_wavelength} for more details.}
    \label{fig:paper3_combined}
\end{figure*}


We also compared the radial brightness profiles to the expected $r^{-2}$ illumination drop-off, typical of scattered light emission, to determine whether the extent of the observed emission is influenced by disc morphology or limited by observational sensitivity (see bottom row of  Fig.~\ref{fig:paper3_profiles_hr4049}, \ref{fig:paper3_profiles_hr4226}, \ref{fig:paper3_profiles_umon}, \ref{fig:paper3_profiles_v709car}, \ref{fig:paper3_profiles_ar_pup} in Appendix~\ref{sec:paper3_ap_profiles}). 
For HR\,4049, HR\,422, and U\,Mon, we found that beyond $\sim 0.03-0.05"$, the radial brightness profiles drop off more steeply than the $r^{-2}$ trend in both the $V-$ and $I'-$bands, suggesting a significant reduction in surface dust density or a shadowing effect beyond this region at the observed wavelengths \citep[e.g.,][]{Perez2018ApJ...869L..50P}. In contrast, V709\,Car profile follows the $r^{-2}$ illumination, indicating sensitivity limitations in fully resolving the disc's surface. For AR\,Pup, the orientation of the system significantly impacts the radial brightness profile, accounting for the deviation from the $r^{-2}$ trend. We discuss possible causes of these effects for each binary system in Section~\ref{sec:paper3_indiv_cases}.



\subsection{Individual case studies}
\label{sec:paper3_indiv_cases}

In this section, we provide a comprehensive analysis of the SPHERE/ZIMPOL polarimetric imaging results for each evolved binary system in our sample. For each target, we present detailed observational findings, including the resolved disc structures and their scattering and polarization properties. We also compare our results, where possible, with previous studies based on high-resolution imaging data, IR and radio interferometry.

\subsubsection{AR\,Pup}
\label{sec:paper3_ar_pup}

AR\,Pup was the first post-AGB binary with its extended disc structure resolved using SPHERE \citep{Ertel2019AJ....157..110E}. However, that study lacked polarimetric data, as the SPHERE polarimetric mode was not available at the time. Here, we present the first multi-wavelength polarimetric results for this target.

Similar to other targets in the sample, the polarimetric images of AR\,Pup include contributions from unresolved central polarization, which arises from both the unresolved portion of the disc and interstellar polarization (see Section~\ref{sec:paper3_data_reduction}). Although we estimated the degree and orientation of the unresolved component (DoLP and AoPL of $2.4\pm0.2$\% and $57\pm2^\circ$ in $V-$band and $3.7\pm0.2$\% and $69\pm2^\circ$ in $I'-$band), the orientation of the disc likely leads to significant overestimation of the unresolved polarized signal. This complicates the subtraction of unresolved polarization without affecting the resolved disc structure. Therefore, we did not apply the correction for unresolved polarization for this data. We note that both the radial and linear brightness profiles of AR\,Pup polarimetric images ($I_{\rm pol}$) exhibit clear peaks at the position of the central binary, corresponding to the unresolved polarization, as well as additional peaks associated with the extended disc polarimetric emission (see Fig.~\ref{fig:paper3_profiles_ar_pup}, Appendix~\ref{sec:paper3_ap_profiles}).

The measured disc brightness in polarized light for AR\,Pup is 4.4$\pm$0.3\% of the total intensity in the $V$-band and 5.1$\pm$0.2\% in the $I'-$band, resulting in a grey polarimetric colour index of $\eta_{VI}=0.4\pm0.3$. AR\,Pup displays the highest polarimetric disc brightness in our sample, likely due to its disc orientation, which partially obscures the host binary and leads to an underestimation of the stellar intensity. This aligns with AR\,Pup's known RVb phenomenon, a long-term periodic variation in mean magnitude \citep{Kiss2007MNRAS.375.1338K}, typically explained by an inclined circumbinary disc that periodically obscures the pulsating primary star. AR\,Pup is the only target in the sample for which the polarimetric disc brightness slightly increases with wavelength. However, this increase may be attributed to the greater number of scattered photons reaching the observer due to the decrease in dust opacity at longer wavelengths \citep{Kirchschlager2014A&A...568A.103K, Tazaki2018ApJ...860...79T}, rather than an increase in polarimetric efficiency. Investigating the deconvolved DoLP map of the resolved scattered emission of AR\,Pup (see bottom panel of Fig.~\ref{fig:paper3_AR_Pup} and Section~\ref{sec:paper3_scatter} for the details) we found a maximum polarization efficiency to be $\sim0.7$ in $V-$band and $\sim0.55$ in $I'-$band, in both cases peak was located to the east from the position of the binary. For the northwestern disc surface, the polarization achieves $\sim0.2$ in $V-$band and $\sim0.3$ in $I'-$band. 

AR\,Pup displays a distinct "double-bowl" structure, separated by a dark band, in both $V-$ and $I'-$band polarimetric images. This feature is more prominent in the $I'-$band. The same shape appears in the total intensity frames (see Section~\ref{sec:paper3_scatter}), and we highlight these substructures in Fig.~\ref{fig:paper3_AR_Pup}. This resolved structure resembles an edge-on flared disc, leading us to interpret the dark band as the optically thick disc mid-plane, with the two "bowls" representing the surfaces of the disc scattering stellar light. From the location of the disc mid-plane in the polarimetric images, we estimate its size to be about 80 mas, with an inclination of $75\pm10^\circ$ and PA of $50\pm5^\circ$.  The southeastern disc surface appears brighter than the northwestern one in both scattered and polarized light, consistent with previous high-resolution imaging of AR\,Pup \citep{Ertel2019AJ....157..110E}. This study suggested that the southeastern surface is oriented toward us, allowing starlight to scatter directly into our line of sight, while the light scattered from the northwestern surface is partially blocked by the disc itself. We agree with this interpretation and argue that this disc orientation explains why the northwestern "bowl" appears significantly dimmer in the azimuthally polarized $Q_\phi$ images compared to the total polarized frames, whereas the southeastern "bowl" remains consistently bright. If the northwestern surface is oriented away from us, the stellar light scattered there likely undergoes multiple scattering through the disc material, disrupting the polarization orientation and reducing the expected azimuthal $Q_\phi$ signal typically seen after single scattering. The suggested disc orientation is further supported by the fact that the northwestern "bowl" is brighter in the $I'-$band than in the $V-$band. This pattern is consistent with the behaviour of light as it passes through the disc, where dust opacity decreases with increasing wavelength, allowing more light to penetrate.


\begin{figure} 
     \includegraphics[width=0.49\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_V_PI_deconv.png}
     \includegraphics[width=0.46\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_I_PI_deconv.png}
     \includegraphics[width=0.49\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_V_I_deconv.png}
     \includegraphics[width=0.47\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_I_I_deconv.png}
     \includegraphics[width=0.5\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_V_DOLP_decon.png}
     \hspace{0.4cm}
     \includegraphics[width=0.47\linewidth]{SourcesPlots/analysis/scattered/AR_Pup_dc_notnorm_I_DOLP_decon.png}

    \caption[Resulting images of AR\,Pup in $V-$ (left column) and $I'-$ (right column) bands.]{Resulting images of AR\,Pup in $V-$ (left column) and $I'-$ (right column) bands. The top row shows total polarized images with highlighted disc midplane (white ellipse) and flared disc scattering surfaces (dashed orange line). The middle row shows deconvolved total intensity images with highlighted disc midplane and scattering surfaces. The bottom row shows a deconvolved  DoLP map (see Section~\ref{sec:paper3_scatter}) with contours marking regions with polarimetric efficiency of 15\% (black), 30\% (white) and 50\% (orange). Polarized and total intensity images are presented on an inverse hyperbolic scale. All images are oriented North up and East to the left. See Section~\ref{sec:paper3_ar_pup} for details.}

    \label{fig:paper3_AR_Pup}
\end{figure}


\subsubsection{HR\,4049}
\label{sec:paper3_hr4049}

HR\,4049 was observed twice, on January 7 and 8, 2019, due to not perfect weather conditions during the first observation. To increase the signal-to-noise ratio, we initially reduced the polarimetric cycles from each observation separately, selecting the highest-quality images before combining them. We then mean-combined all frames after reduction and performed the analysis on the combined set.

We measured the degree and orientation of the unresolved component (DoLP and AoPL of $0.11\pm0.07$\% and $57\pm25^\circ$ in $V-$band and $0.23\pm0.04$\% and $63\pm9^\circ$ in $I'-$band), finding it to be the smallest in the sample (see Section~\ref{sec:paper3_data_reduction}). This can be attributed to HR\,4049's position above the Galactic midplane, which reduces polarization from the diffuse interstellar medium along the line of sight. Additionally, the angular size of the disc dust inner rim, as resolved with near-IR interferometry \citep[$\sim16$ mas, ][]{Kluska2019A&A...631A.108K}, suggests that the unresolved portion of the disc is relatively small. Moreover, the unresolved central polarization we measured for HR\,4049 falls within the uncertainty range of the total polarization detected from the reference star (HD96314), both in value and orientation. Therefore, we conclude that the unresolved central polarization observed for HR\,4049 is predominantly caused by interstellar polarization rather than the unresolved portion of the circumbinary disc.

We measured the resolved disc brightness in polarized light of HR\,4049 to be 1.1$\pm$0.3\% of the total intensity in the $V$-band and 0.95$\pm$0.1\% in the $I'-$band, resulting in a borderline blueish polarimetric colour index of $\eta_{VI}=-0.4\pm1$ and $\eta_{VH}=0.6\pm0.5$. The unusually large uncertainty in $\eta_{VI}$ is primarily due to a ‘cross-shaped’ observational artefact in polarimetric intensity observed in the $V-$ and (to less extent) $I'-$bands (see Section~\ref{sec:paper3_data_reduction}), which we attribute to an instrumental effect rather than a physical feature. This intensity drop also disrupts the azimuthal brightness profiles in both $V-$ and $I'-$bands (see Fig.~\ref{fig:paper3_profiles_hr4049}, Appendix~\ref{sec:paper3_ap_profiles}).  

HR\,4049 shows a clear bright 'ring' in both $V-$ and $I'-$bands. We obtained a disc inclination of $29^\circ$  and $23^\circ$, with PA of $109^\circ$ and $138^\circ$ in $V-$ and $I'-$bands, respectively (see Section~\ref{sec:paper3_disc_orient}). These values align with previously identified disc orientations in near-IR $H$-band polarimetric imaging \citep[inclination of $17^\circ$ and PA of $174^\circ$,][]{Andrych2023MNRAS.524.4168A}, suggesting a nearly face-on disc orientation. However, this low inclination contradicts the observed RVb phenomenon of the HR\,4049 \citep{Waelkens1991A&A...242..433W} and also differs from the results of IR interferometric studies \citep[inclination of 49$^\circ$, PA of 63$^\circ$,][]{Kluska2019A&A...631A.108K}. While we cannot fully explain this discrepancy, we propose that the RVb phenomenon may be caused by a potentially misaligned inner part of the disc or other unresolved dynamical processes closer to the central binary. We did not detect any significant change in the size of the resolved disc of HR\,4049 across the $V-$, $I'-$, and $H$-band polarimetric data, with extended resolved emission observed up to $\sim80$ mas from the central star (see Fig.~\ref{fig:paper3_combined}). We found that in both $V$ and $I'-$bands, starting from $\sim 0.04"$, the radial brightness profiles decrease more steeply than the expected r$^{-2}$ illumination drop-off (see Fig.~\ref{fig:paper3_profiles_hr4049}, Appendix~\ref{sec:paper3_ap_profiles}). This suggests that the observed disc size is determined by disc morphology rather than by observational sensitivity. Although the $V-$ and $H-$band polarimetric images do not reveal any significant substructures, the $I'-$band images display a clear arc-like feature to the northeast of the binary position. To determine whether this substructure might be an observational artefact, we compared separately reduced observations from January 7 and 8, 2019, and found that this structure is consistently visible in both datasets. While additional observations of the disc midplane, such as dust continuum observations with ALMA, are necessary to draw definitive conclusions about the physics of this feature, we speculate that it may be part of a spiral structure.


\subsubsection{HR\,4226}
\label{sec:paper3_hr4226}

HR\,4226 is located in the Galactic plane; however, we measured a relatively low degree of unresolved polarization for this target, with DoLP of $0.15\pm0.06$\% in $V-$band and $0.16\pm0.04$\% in $I'-$band (see Section~\ref{sec:paper3_data_reduction}). Although the degree of unresolved polarization is similar to that detected from the reference star (HD98025), the orientation differs (see Fig.~\ref{fig:paper3_wave_dep_unres}). Thus, we cannot determine the relative contribution of the unresolved circumbinary disc polarization and interstellar polarization for HR\,4226.

For the resolved disc brightness in polarized light of HR\,4226, we measured  1.9$\pm$0.1\% of the total intensity in the $V$-band and 1.75$\pm$0.06\% in the $I'-$band, resulting in a grey polarimetric colour index of $\eta_{VI}=-0.3\pm0.2$. We also note that similarly to HR\,4049 (see Section~\ref{sec:paper3_hr4049}), the $V$-band polarimetric observations of HR\,4226 suffer from reduction artefact. Although the effect is less pronounced, it causes a ‘cross-shaped’ intensity decrease that disrupts the azimuthal brightness profile of the disc (see Fig.~\ref{fig:paper3_profiles_hr4049} and Section~\ref{sec:paper3_data_reduction}).  

HR\,4226 shows a clear bright 'ring' in both $V-$ and $I'-$bands. We estimated a disc inclination of $51^\circ$  and $40^\circ$, with PA of $104^\circ$ and $106^\circ$ in $V-$ and $I'-$bands, respectively (see Section~\ref{sec:paper3_disc_orient}). We did not detect any significant change in the size of the resolved disc of HR\,4226 across the $V$-, $I'-$band polarimetric data with the extended emission of up to $\sim90$ mas from the central star (see Fig.~\ref{fig:paper3_combined}). These findings complement geometric modelling results of mid-IR interferometric data from VLT/MIDI \citep{Hillen2017}, shown as white contours in the same image. We also found that in both $V-$ and $I'-$bands, starting from $\sim 0.03"$, the radial brightness profiles decrease more steeply than the expected r$^{-2}$ illumination drop-off (see bottom panel of Fig.~\ref{fig:paper3_profiles_hr4226}, Appendix~\ref{sec:paper3_ap_profiles}). This suggests that the observed disc size is determined by disc morphology rather than by observational sensitivity.  We also note that azimuthal brightness profiles of the disc show two distinct peaks along the major axis (see middle panel of Fig.~\ref{fig:paper3_profiles_hr4226}, Appendix~\ref{sec:paper3_ap_profiles}), commonly attributed to the projection of an inclined circular disc onto the sky.


\subsubsection{U\,Mon}
\label{sec:paper3_umon}

For U\,Mon, we measured an unresolved polarization degree of $0.52\pm0.05$\% in the $V$-band and $0.77\pm0.04$\% in the $I'$-band, both of which exceed the polarized intensity measured for the reference star (see Fig.~\ref{fig:paper3_wave_dep_unres}). Since U\,Mon is located in the Galactic plane, we expect a quite significant effect of interstellar polarization for this system (see Section~\ref{sec:paper3_data_reduction}). However, the reference star HD71253 lies above the Galactic midplane and, therefore, cannot serve as a reliable estimate of interstellar polarization for U\,Mon. Therefore, we cannot determine the relative contributions of the unresolved circumbinary disc polarization and interstellar polarization for U\,Mon.

We measured polarized disc brightness of U\,Mon to be 1.8$\pm$0.2\% of the total intensity in the $V$-band and 1.4$\pm$0.07\% in the $I'-$band, resulting in a blueish polarimetric colour index of $\eta_{VI}=-0.6\pm0.4$ and $\eta_{VH}=-0.9\pm0.3$. 

U\,Mon shows a clear bright 'ring' in  $V-$band and two arcs separated by a dark strip in $I'-$band. However, we note that this darker area is an artefact from the subtraction of unresolved central polarization, which also includes some polarized emission from the disc. We estimated a disc inclination of $\sim 45^\circ$  and PA of $\sim130^\circ$ in both $V-$ and $I'-$bands (see Section~\ref{sec:paper3_disc_orient}). While the PA of the disc aligns with the previously identified value from near-IR $H$-band polarimetric imaging ($\sim140^\circ$), our inclination estimate is significantly higher \citep[previously estimated at $25^\circ$ in the $H$-band,][]{Andrych2023MNRAS.524.4168A}. However, the higher inclination value based on $V-$ and $I'-$band data is consistent with values obtained from geometric modelling using near-IR interferometric observations \citep{Kluska2019A&A...631A.108K} and with the observed long-term periodic variation in mean magnitude \citep[RVb phenomenon,][]{Kiss2017}. This phenomenon is commonly attributed to an inclined circumbinary disc that intermittently obscures the pulsating primary star during certain phases of its orbit \citep{Vega2017ApJ...839...48V, Manick2017, Kiss2017}. We note that the north-western side of the disc appears brighter than other areas in both the $V$- and $I'$-bands (see Fig.~\ref{fig:paper3_profiles_umon}). We suggest that this brightness peak is likely caused by the forward scattering of stellar light on dust grains that are comparable in size to the observational wavelength \citep[e.g.,][]{Ginski2023ApJ...953...92G}. This effect also indicates that the northern part of the disc is inclined toward the observer.

While we do not observe any significant change in the resolved disc size or morphology across the $V$- and $I'$-band polarimetric data, we note that the near-IR $H$-band polarimetric image reveals a more extended disc (see Fig.~\ref{fig:paper3_combined}). A similar effect has been reported for the post-AGB system IRAS\,08544-4431 \citep{Andrych2024IRAS08}. As suggested for IRAS\,08544-4431, we propose that the larger apparent disc size and lower estimated inclination in $H$-band polarimetric images may result from SPHERE probing slightly deeper disc layers at longer wavelengths, as dust opacity decreases from optical to near-IR \citep{Kirchschlager2014A&A...568A.103K, Tazaki2018ApJ...860...79T}.


\subsubsection{V709\,Car}
\label{sec:paper3_v709_car}

For V709\,Car, we measured a high degree of unresolved polarization with DoLP of $1.7\pm0.16$\% in $V-$band and $2.6\pm0.01$\% in $I'-$band (see Section~\ref{sec:paper3_data_reduction}). These values are much higher than polarization detected from the reference star HD94680, which is located closely in the Galactic plane. Therefore, we suggest that the unresolved central polarization measured for V709\,Car is predominantly caused by the unresolved part of the circumbinary disc rather than polarization in the diffuse interstellar medium along the line of sight.

We measured the resolved disc brightness in polarized light of V709\,Car to be the smallest in the sample with 0.6$\pm$0.09\% of the total intensity in the $V$-band and 0.49$\pm$0.07\% in the $I'-$band, resulting in a borderline blueish polarimetric colour index of $\eta_{VI}=-0.52\pm0.76$. We also note that similarly to HR\,4049 and HR\,4226 (see Section~\ref{sec:paper3_hr4049}), the polarimetric observations of HR\,4226 suffer from instrumental artefacts that disrupt the azimuthal brightness profile of the disc (see Fig.~\ref{fig:paper3_profiles_v709car} and Section~\ref{sec:paper3_data_reduction}). However, this effect is visible only in $I'$-band data. 

Similar to other targets in the sample, V709\,Car also shows a 'ring' structure in both $V-$ and $I'-$bands, which we interpret as a circumbinary disc surface. We estimated a disc inclination of $\sim30^\circ$  and PA of $\sim120^\circ$ in both $V-$ and $I'-$bands (see Section~\ref{sec:paper3_disc_orient}).  We also note that $V-$band azimuthal brightness profile of the disc shows two distinct peaks along the major axis (see middle panel of Fig.~\ref{fig:paper3_profiles_v709car}, Appendix~\ref{sec:paper3_ap_profiles}), commonly attributed to the projection of an inclined circular disc onto the sky. V709\,Car is the only target in our sample that shows a significant difference in the size of the resolved extended emission in reaching $\sim150$ mas from the central star in $I'$-band polarimetric image, while appearing much smaller in $V-$band (see Fig.~\ref{fig:paper3_substr}). However, we note that due to the low level of resolved signal, these values have to be treated with caution. We also found that in both $V$ and $I'-$bands, the radial brightness profiles follows the expected r$^{-2}$ illumination drop-off (see bottom panel of Fig.~\ref{fig:paper3_profiles_hr4226}, Appendix~\ref{sec:paper3_ap_profiles}). This suggests that the observed disc size is determined by observational sensitivity rather than disc morphology. These findings complement geometric modelling results of mid-IR interferometric data from VLT/MIDI \citep{Hillen2017}, shown as a white contour in Fig.~\ref{fig:paper3_combined}.
 

\section{Discussion}
\label{sec:paper3_discussion}

In this section, we interpret the obtained results to better understand the morphology and dust characteristics in post-AGB circumbinary discs. We accomplish this by: i) characterizing the dust properties on the disc surfaces within our sample, ii) comparing the circumstellar environments of AGB and post-AGB systems, and iii) examining the similarities between circumbinary discs around post-AGB binaries and PPDs around YSOs.


\subsection{Characterizing the dust properties and disc morphology of post-AGB binaries}

The appearance of circumstellar discs in scattered light depends on their geometry and the optical properties of the dust particles within them. These characteristics can be inferred by analyzing the intensity and polarization degree of reflected stellar light, as well as its brightness distribution and wavelength dependencies \citep[e.g.,][]{Tazaki2023ApJ...944L..43T, Garufi2018A&A...620A..94G}.

All post-AGB systems in our sample (AR\,Pup, HR\,4049, HR\,4226, and U\,Mon) exhibit high polarimetric disc brightness, with more than 1\% of the total intensity of the system in optical wavelengths ($V$ and $I'$-bands). For AR\,Pup, we directly measured the polarization efficiency by analyzing the deconvolved DoLP map of the resolved scattered light emission. We found a maximum polarization efficiency of $\sim0.7$ in the $V-$band and $\sim0.55$ in the $I'-$band. We also note that U\,Mon shows a forward scattering peak, which mirrors similar findings for the post-AGB system IRAS\,08544-4431 \citep{Andrych2024IRAS08} and is indicative of anisotropic scattering. However, forward scattering signatures are less evident for HR\,4049 and HR\,4226, likely due to their orientation, instrumental artefacts, and limited spatial resolution. The polarimetric colour across the sample tends toward grey or slightly blue, except for AR\,Pup, which exhibits a borderline grey-red colour. In AR\,Pup, total polarimetric brightness increases with wavelength, likely due to dominant dust absorption effects caused by the high inclination of the system and significant disc flaring (see Fig~\ref{fig:paper3_AR_Pup}). 

Numerical models by \citet{Tazaki2019MNRAS.485.4951T} suggest that high polarization efficiency, presence of forward scattering, and grey or blue polarimetric disc colours arise from porous aggregates composed of small monomers. Furthermore, radiative transfer (RT) models by Min (2012) illustrate that polarimetric intensity distributions in inclined discs with porous dust grains align well with the polarimetric morphology observed in AR\,Pup disc. Based on these comparisons, we suggest the presence of large (submicron-sized) porous dust aggregates on the surfaces of studied post-AGB circumbinary discs.

Polarimetric imaging of all observed post-AGB systems reveals a bright central disc region and more extended emission with resolved substructures in both $V-$ and $I'-$bands. We note that substructures appear brighter in the $I'-$band. A comparison with SPHERE/IRDIS near-IR imaging results shows that U\,Mon shows a larger disc size in near-IR compared to optical, similar to IRAS\,08544-4431 \citep{Andrych2024IRAS08}. In contrast, HR\,4049's disc size remains consistent across wavelengths. These variations and a range of resolved substructures in the post-AGB discs suggest a diversity in disc geometry and potentially dust composition within our sample. Additionally, we note that all targets studied with SPHERE in multi-wavelength polarimetric imaging to date belong to the "full" disc category (with dust inner rims located at the theoretical dust sublimation radius). To thoroughly investigate the dust properties and geometry of post-AGB circumbinary discs, future multi-wavelength polarimetric imaging observations should also include "transition" discs, which contain large inner cavities.

\subsection{Comparing the circumstellar environments of AGB and post-AGB binaries}

 We observe that the resolved polarized emission of V709\,Car, one of the targets in our sample, appears more clumpy and less confined compared to other post-AGB systems. These characteristics suggest the potential presence of ongoing stellar wind-driven mass loss and extended circumstellar material rather than a dense, compact disc. The significantly lower effective temperature of the primary star, compared to typical post-AGB stars, raises the possibility that V709\,Car may be less evolved and could still be in the AGB stage \citep[see Section~\ref{sec:paper3_target},][]{Kluska2022}. Our findings for V709\,Car are consistent with recent studies of AGB star circumstellar environments. For instance, a recent SPHERE/ZIMPOL study by \citet{Montarges2023A&A...671A..96M}, which observed a sample of 14 AGB stars, revealed that their dusty circumstellar environments are predominantly clumpy with isolated dust features. Additionally, polarimetric observations of the highly inclined AGB binary system L2 Pup \citep{Kervella2015EAS....71..211K} show a configuration remarkably similar to that observed in the post-AGB binary AR\,Pup in this study. Both targets exhibit extremely flared outflows that are perpendicular to the disc midplane.

These findings highlight the need for a consistent and detailed study of the circumstellar environments of post-AGB stars, together with AGB stars and planetary nebulae. Such research would allow us to probe ambient environments with varying conditions and enhance our understanding of dust formation and processing, as well as the roles of stellar parameters and binarity in shaping the dusty circumstellar medium.


\subsection{Comparison of discs around post-AGBs with protoplanetary discs around YSOs}

Post-AGB circumbinary discs and PPDs exhibit remarkable similarities despite their different formation histories and lifetimes (see Section~\ref{sec:paper3_intro}). Our findings demonstrate a consistent optical and near-IR polarized brightness level relative to stellar intensity  ($\sim10^{-2}$) in post-AGB circumbinary discs, placing them among the brightest PPDs \citep{Avenhaus2018ApJ...863...44A, Ma2024A&A...683A..18M}. Although PPDs around YSOs typically show grey to red polarimetric colours, our observations reveal comparable wavelength-dependent polarimetric behaviour between post-AGB circumbinary discs and certain PPDs, such as those around T Tauri stars like TW Hya, PDS 70, and PDS 66 \citep{Ma2024A&A...683A..18M}. The complex morphologies observed in post-AGB circumbinary discs, including arcs, gaps, cavities, and flared disc surfaces \citep[this study; see also][]{Ertel2019AJ....157..110E, Andrych2023MNRAS.524.4168A, Andrych2024IRAS08}, also resemble structures found in protoplanetary discs. Although post-AGB systems are generally more distant, which limits spatial resolution compared to YSOs, these striking similarities strengthen the idea that post-AGB circumbinary discs share structural and possibly evolutionary characteristics with protoplanetary discs. This connection highlights the relevance of studying post-AGB systems to gain insights into disc evolution across various stellar environments.

\section{Conclusions}
\label{sec:paper3_conclusion}

We present a multi-wavelength polarimetric imaging study of five post-AGB binary systems (AR\,Pup, HR\,4049, HR\,4226, U\,Mon, and V709\,Car) using the VLT/SPHERE instrument. Our study aimed to i) assess whether the polarimetric properties and surface morphologies of circumbinary discs are consistent across the post-AGB sample, ii) explore the dust properties inferred from both the intensity and degree of polarization of the scattered light and iii) compare our findings with known observations for AGB and YSO systems.

Our results reveal resolved, complex disc morphologies for all post-AGB targets in polarized light in optical $V-$ and $I'-$bands. All post-AGBs exhibit high polarimetric disc brightness, with more than 1\% of the total intensity. For post-AGB binary AR\,Pup, we also resolved circumbinary disc in scattered light and directly measured the maximum polarization efficiency of $\sim0.7$ in the $V-$band and $\sim0.55$ in the $I'-$band. The polarimetric colour across the sample tends toward grey or slightly blue, except for AR\,Pup, which exhibits a borderline grey-red colour (likely due to dominant dust absorption effects caused by the high inclination of the system and significant disc flaring). The high polarization efficiency, grey or blue polarimetric colours, and polarimetric intensity distribution observed in post-AGB circumbinary discs align with theoretical models of porous aggregates composed of small monomers as the dominant surface dust composition. Comparing our results with those from SPHERE/IRDIS near-IR imaging reveals that U\,Mon has a larger disc size in the near-IR compared to the optical, similar to IRAS\,08544-4431 \citep{Andrych2024IRAS08}. In contrast, the disc size of HR\,4049 remains consistent across wavelengths. These variations, along with the diverse resolved substructures in the post-AGB discs, indicate a variety of disc geometries and potentially different dust compositions within our sample. 

We also note that V709\,Car exhibits more clumpy and less confined resolved polarized emission compared to other post-AGB systems. This aligns with the suggestion that V709\,Car may be less evolved, with its primary star potentially still in the AGB evolutionary stage, characterized by strong stellar winds and a high mass-loss rate. The resolved size of the polarimetric emission for V709\,Car also appears significantly larger in the $I'$-band compared to the $V$-band. We suggest that this wavelength-dependent morphology may result from disc self-shadowing effects due to higher dust absorption at shorter wavelengths. These findings highlight the need for a comprehensive study of the circumstellar environments of post-AGB stars, AGB stars, and planetary nebulae to better understand the processes involved in dust formation and evolution in evolved systems.

Additionally, our findings reinforce previously identified similarities between post-AGB circumbinary discs and PPDs around YSOs. These include complex disc morphologies,  high polarimetric brightness, comparable wavelength-dependence of polarized emission, dust size and compositions. These similarities highlight the importance of post-AGB systems in enhancing our understanding of disc evolution across various stellar environments. A comprehensive approach that integrates multi-wavelength and multi-technique observations with advanced radiative-transfer modelling will further clarify disc dynamics and evolution in these systems and enhance our understanding of the roles of stellar parameters and binarity in shaping the dusty circumstellar medium and facilitating potential planet formation.

\section*{Acknowledgements}

DK and KA acknowledge the support of the Australian Research Council (ARC) Discovery Early Career Research Award (DECRA) grant (DE190100813). This research was supported in part by the Australian Research Council Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D) through project number CE170100013. J.K. acknowledges support from FWO under the senior postdoctoral fellowship (1281121N). This study is based on observations collected at the European Southern Observatory under ESO programmes 101.D-0752(A), 0102.D-0696(A), and 0101.D-0807(B). This work has made use of the High Contrast Data Centre, jointly operated by OSUG/IPAG (Grenoble), PYTHEAS/LAM/CeSAM (Marseille), OCA/Lagrange (Nice), Observatoire de Paris/LESIA (Paris), and Observatoire de Lyon/CRAL, and supported by a grant from Labex OSUG@2020 (Investissements d’avenir – ANR10 LABX56). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Data Availability}
The data underlying this article are stored online in the ESO Science Archive Facility at http://archive.eso.org, and can be accessed by program IDs.


==> scratch.tex <==

HR4226
 A near-IR interferometric study with VLTI/PIONIER found that the circumbinary material was over-resolved, resulting in a binary model without a detectable ring \citep{Kluska2019A&A...631A.108K}. Geometric modelling of mid-IR interferometric data from VLT/MIDI revealed a ring-like structure, with a half-light radius of $18\pm1$ mas and an outer diameter of $58\pm3$ mas \citep{Hillen2017}. 
Radial velocity monitoring indicates an orbital period of $527\pm6$ days with small velocity variations ($\Delta V \simeq 1$ km/s), leading to an exceptionally low mass function of $1.4\times10^{-6}$ \citep{Maas2003PhDT.......265M}.
Radial velocity monitoring for this target found orbital period of 527+-6 days and mass function of f(M) 1.4*10^(-6) Their results indicate an orbital period of 527+-6 days and very small radial velocity variations (ΔV ≈ 1 km/s), which results in a exceptionally small estimate for the companion mass (Assuming a 0.6 M☉ primary and considering different inclinations, they estimate a companion mass around 0.008 M☉  i.e., around 8 Jupiter masses.).
low companion mass estimate of $\sim$8 Jupiter masses, assuming a 0.6 M$_\odot$ primary.  This is concerning because typical companion for post-AGb star  is 1 solar mass + orbital distribution (Omen paper). So those is exceptional kind of a system. While its period of $\sim$500 days suggests that radial velocity variations could be caused by pulsations in the Mira regime, its RV amplitude is significantly weaker than that of classical Mira variables.  This brings the question the AGB nature for the star based on the amplitude. 
 
 HR 4226 exhibits high polarimetric brightness (>1.5\%) and a well-defined disc surface (see Table~\ref{tab:paper3_disc_orient} and Fig.\ref{fig:paper3_reduced}). Given its very small radial velocity variations \citep[ΔV ≈ 1 km/s,][]{Maas2003A&A...405..271M} and the uncertainty in its effective temperature, this system may resemble an L$_2$ Pup-type system, where an AGB star is observed with a substellar companion or a planet.










A recent SPHERE/ZIMPOL study by \citet{Montarges2023A&A...671A..96M}, which observed a sample of 14 single AGB stars, revealed that their dusty circumstellar environments are predominantly clumpy with isolated dust features. They also showed that observed poalrization efficiency decreasing with wavelength and does not exceeds $\sim$40\%. They also showed that the grains seem either small (0.01−0.1 μm) or possibly intermediate sized (0.01−1 μm). 
 
Polarimetric observations of the highly inclined AGB binary system L2 Pup \citep{Kervella2015EAS....71..211K} show that in precense of (sub)stellar companion, intermediate mass stars can host dusty disc already during the AGB phase. They also found maximum polarisation efficiency of 0.46 in $V$-band and 0.61 in $R$-band. We note that a configuration of L2 Pup disc is remarkably similar to that observed in the post-AGB binary AR\,Pup in this study. Both targets exhibit extremely flared outflows that are perpendicular to the disc midplane. However, AR\,Pup shows higher polarisation efficiency ($\sim0.7$ in the $V-$band and $\sim0.55$ in the $I'-$band) that decrease with wavelength, contrary to the increase for L2 Pup. 

These Diffrerences in polarisation efficiency for AGB and post-AGB circumbinary discs suggest larger or more porous dust aggregates present on the poat-AGB disc surface. 

 
We found that as a sample post-AGB circumbinary discs show much higher polarimetric efficiency ($\sim0.7$ in the $V-$band and $\sim0.55$ in the $I'-$band) and larger grain sizes than what was found for AGB stars while also show nearly constant or slightly decreesing polarised brightness with wavelength.
However, For one target  V709\,Car, We found lower resolved polarized brigtnses and less confined resolved polarised emmission compared to other post-AGB systems (see Section~\ref{sec:paper3_v709_car}). These characteristics suggest the potential presence of ongoing stellar wind-driven mass loss and extended circumstellar material rather than a dense, compact disc. The lower effective temperature of the primary star, compared to typical post-AGB stars, raises the possibility that V709\,Car may be less evolved and could still be in the AGB stage \citep[see Section~\ref{sec:paper3_target},][]{Kluska2022}. 
We note that the effective temperature T$_{\rm eff}$ derived from SED fitting for V709\,Car is $3500\pm175$ K, suggesting that this M-type star is too cool for a post-AGB object and may still be in the AGB phase \citep{Hillen2017, Kluska2022}. While our polarimetric imaging results do not show significant differences between V709\,Car and the other post-AGB systems in our sample, we note that AGB stars with companions are also known to host circumstellar discs \citep[e.g.,][]{Kervella2015A&A...578A..77K}. Therefore, a detailed spectroscopic analysis is required to accurately determine its evolutionary stage.

 This result further highlight a question of how fast a stable circumbinary disc can be formed in evolved binary systems.  

These findings highlight the need for a consistent and detailed study of the circumstellar environments of post-AGB stars, together with AGB stars and planetary nebulae. Such research would allow us to probe ambient environments with varying conditions and enhance our understanding of dust formation and processing, as well as the roles of stellar parameters and binarity in shaping the dusty circumstellar medium.












%%%%%%%%%%NEW








